Complete measurement of $\Lambda$ electromagnetic form factors

The exclusive process $e^+e^-\rightarrow\Lambda\bar{\Lambda}$, with $\Lambda \to p\pi^-$ and $\bar{\Lambda} \to \bar{p}\pi^+$, has been studied at $\sqrt{s} =$ 2.396 GeV for measurement of the $\Lambda$ electric and magnetic form factors, $G_E$ and $G_M$. A data sample, corresponding to an integrated luminosity of 66.9 pb$^{-1}$, was collected with the BESIII detector for this purpose. A multi-dimensional analysis with a complete decomposition of the spin structure of the reaction enables a determination of the modulus of the ratio $R=|G_E/G_M|$ and, for the first time for any baryon, the relative phase $\Delta\Phi=\Phi_E-\Phi_M$. The resulting values are obtained using the recent and most precise measured value of the asymmetry parameter $\alpha_{\Lambda}$ = $0.750~\pm~0.010$ to be $R~=~0.96\pm0.14~(\rm stat.)\pm~0.02~(\rm sys.)$ and $\Delta\Phi=37^{\mathrm{o}}\pm~12^{\mathrm{o}}~(\rm stat.)\pm~6^{\mathrm{o}}~(\rm sys.)$, respectively. In addition, the cross section is measured with unprecedented precision to be $\sigma = 118.7~\pm~5.3~(\rm stat.)\pm~5.1~(\rm sys.)$ pb, which corresponds to an effective form factor of $|G|=0.123~\pm~0.003~(\rm stat.)\pm~0.003~(\rm sys.)$. The contribution from two-photon exchange is found to be negligible. Our result enables the first complete determination of baryon time-like electromagnetic form factors.

==> authors2018-12-21.tex <==
%\author{Author list}
\begin{small}
\begin{center}
M.~Ablikim$^{1}$, M.~N.~Achasov$^{10,d}$, P.~Adlarson$^{59}$, S. ~Ahmed$^{15}$, M.~Albrecht$^{4}$, M.~Alekseev$^{58A,58C}$, A.~Amoroso$^{58A,58C}$, F.~F.~An$^{1}$, Q.~An$^{55,43}$, Y.~Bai$^{42}$, O.~Bakina$^{27}$, R.~Baldini Ferroli$^{23A}$, Y.~Ban$^{35}$, K.~Begzsuren$^{25}$, J.~V.~Bennett$^{5}$, N.~Berger$^{26}$, M.~Bertani$^{23A}$, D.~Bettoni$^{24A}$, F.~Bianchi$^{58A,58C}$, J.~Biernat$^{59}$, J.~Bloms$^{52}$, I.~Boyko$^{27}$, R.~A.~Briere$^{5}$, H.~Cai$^{60}$, X.~Cai$^{1,43}$, A.~Calcaterra$^{23A}$, G.~F.~Cao$^{1,47}$, N.~Cao$^{1,47}$, S.~A.~Cetin$^{46B}$, J.~Chai$^{58C}$, J.~F.~Chang$^{1,43}$, W.~L.~Chang$^{1,47}$, G.~Chelkov$^{27,b,c}$, D.~Y.~Chen$^{6}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,47}$, J.~C.~Chen$^{1}$, M.~L.~Chen$^{1,43}$, S.~J.~Chen$^{33}$, Y.~B.~Chen$^{1,43}$, W.~Cheng$^{58C}$, G.~Cibinetto$^{24A}$, F.~Cossio$^{58C}$, X.~F.~Cui$^{34}$, H.~L.~Dai$^{1,43}$, J.~P.~Dai$^{38,h}$, X.~C.~Dai$^{1,47}$, A.~Dbeyssi$^{15}$, D.~Dedovich$^{27}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{26}$, I.~Denysenko$^{27}$, M.~Destefanis$^{58A,58C}$, F.~De~Mori$^{58A,58C}$, Y.~Ding$^{31}$, C.~Dong$^{34}$, J.~Dong$^{1,43}$, L.~Y.~Dong$^{1,47}$, M.~Y.~Dong$^{1,43,47}$, Z.~L.~Dou$^{33}$, S.~X.~Du$^{63}$, J.~Z.~Fan$^{45}$, J.~Fang$^{1,43}$, S.~S.~Fang$^{1,47}$, Y.~Fang$^{1}$, R.~Farinelli$^{24A,24B}$, L.~Fava$^{58B,58C}$, F.~Feldbauer$^{4}$, G.~Felici$^{23A}$, C.~Q.~Feng$^{55,43}$, M.~Fritsch$^{4}$, C.~D.~Fu$^{1}$, Y.~Fu$^{1}$, Q.~Gao$^{1}$, X.~L.~Gao$^{55,43}$, Y.~Gao$^{56}$, Y.~Gao$^{45}$, Y.~G.~Gao$^{6}$, Z.~Gao$^{55,43}$, B. ~Garillon$^{26}$, I.~Garzia$^{24A}$, E.~M.~Gersabeck$^{50}$, A.~Gilman$^{51}$, K.~Goetzen$^{11}$, L.~Gong$^{34}$, W.~X.~Gong$^{1,43}$, W.~Gradl$^{26}$, M.~Greco$^{58A,58C}$, L.~M.~Gu$^{33}$, M.~H.~Gu$^{1,43}$, S.~Gu$^{2}$, Y.~T.~Gu$^{13}$, A.~Q.~Guo$^{22}$, L.~B.~Guo$^{32}$, R.~P.~Guo$^{36}$, Y.~P.~Guo$^{26}$, A.~Guskov$^{27}$, S.~Han$^{60}$, X.~Q.~Hao$^{16}$, F.~A.~Harris$^{48}$, K.~L.~He$^{1,47}$, F.~H.~Heinsius$^{4}$, T.~Held$^{4}$, Y.~K.~Heng$^{1,43,47}$, Y.~R.~Hou$^{47}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,47}$, J.~F.~Hu$^{38,h}$, T.~Hu$^{1,43,47}$, Y.~Hu$^{1}$, G.~S.~Huang$^{55,43}$, J.~S.~Huang$^{16}$, X.~T.~Huang$^{37}$, X.~Z.~Huang$^{33}$, N.~Huesken$^{52}$, T.~Hussain$^{57}$, W.~Ikegami Andersson$^{59}$, W.~Imoehl$^{22}$, M.~Irshad$^{55,43}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{16}$, X.~B.~Ji$^{1,47}$, X.~L.~Ji$^{1,43}$, H.~L.~Jiang$^{37}$, X.~S.~Jiang$^{1,43,47}$, X.~Y.~Jiang$^{34}$, J.~B.~Jiao$^{37}$, Z.~Jiao$^{18}$, D.~P.~Jin$^{1,43,47}$, S.~Jin$^{33}$, Y.~Jin$^{49}$, T.~Johansson$^{59}$, N.~Kalantar-Nayestanaki$^{29}$, X.~S.~Kang$^{31}$, R.~Kappert$^{29}$, M.~Kavatsyuk$^{29}$, B.~C.~Ke$^{1}$, I.~K.~Keshk$^{4}$, T.~Khan$^{55,43}$, A.~Khoukaz$^{52}$, P. ~Kiese$^{26}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{11}$, L.~Koch$^{28}$, O.~B.~Kolcu$^{46B,f}$, B.~Kopf$^{4}$, M.~Kuemmel$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{59}$, M.~Kurth$^{1}$, M.~ G.~Kurth$^{1,47}$, W.~K\"uhn$^{28}$, J.~S.~Lange$^{28}$, P. ~Larin$^{15}$, L.~Lavezzi$^{58C}$, H.~Leithoff$^{26}$, T.~Lenz$^{26}$, C.~Li$^{59}$, Cheng~Li$^{55,43}$, D.~M.~Li$^{63}$, F.~Li$^{1,43}$, F.~Y.~Li$^{35}$, G.~Li$^{1}$, H.~B.~Li$^{1,47}$, H.~J.~Li$^{9,j}$, J.~C.~Li$^{1}$, J.~W.~Li$^{41}$, Ke~Li$^{1}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, P.~L.~Li$^{55,43}$, P.~R.~Li$^{30}$, Q.~Y.~Li$^{37}$, W.~D.~Li$^{1,47}$, W.~G.~Li$^{1}$, X.~H.~Li$^{55,43}$, X.~L.~Li$^{37}$, X.~N.~Li$^{1,43}$, X.~Q.~Li$^{34}$, Z.~B.~Li$^{44}$, Z.~Y.~Li$^{44}$, H.~Liang$^{1,47}$, H.~Liang$^{55,43}$, Y.~F.~Liang$^{40}$, Y.~T.~Liang$^{28}$, G.~R.~Liao$^{12}$, L.~Z.~Liao$^{1,47}$, J.~Libby$^{21}$, C.~X.~Lin$^{44}$, D.~X.~Lin$^{15}$, Y.~J.~Lin$^{13}$, B.~Liu$^{38,h}$, B.~J.~Liu$^{1}$, C.~X.~Liu$^{1}$, D.~Liu$^{55,43}$, D.~Y.~Liu$^{38,h}$, F.~H.~Liu$^{39}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, H.~B.~Liu$^{13}$, H.~M.~Liu$^{1,47}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{17}$, J.~B.~Liu$^{55,43}$, J.~Y.~Liu$^{1,47}$, K.~Y.~Liu$^{31}$, Ke~Liu$^{6}$, Q.~Liu$^{47}$, S.~B.~Liu$^{55,43}$, T.~Liu$^{1,47}$, X.~Liu$^{30}$, X.~Y.~Liu$^{1,47}$, Y.~B.~Liu$^{34}$, Z.~A.~Liu$^{1,43,47}$, Zhiqing~Liu$^{37}$, Y. ~F.~Long$^{35}$, X.~C.~Lou$^{1,43,47}$, H.~J.~Lu$^{18}$, J.~D.~Lu$^{1,47}$, J.~G.~Lu$^{1,43}$, Y.~Lu$^{1}$, Y.~P.~Lu$^{1,43}$, C.~L.~Luo$^{32}$, M.~X.~Luo$^{62}$, P.~W.~Luo$^{44}$, T.~Luo$^{9,j}$, X.~L.~Luo$^{1,43}$, S.~Lusso$^{58C}$, X.~R.~Lyu$^{47}$, F.~C.~Ma$^{31}$, H.~L.~Ma$^{1}$, L.~L. ~Ma$^{37}$, M.~M.~Ma$^{1,47}$, Q.~M.~Ma$^{1}$, X.~N.~Ma$^{34}$, X.~X.~Ma$^{1,47}$, X.~Y.~Ma$^{1,43}$, Y.~M.~Ma$^{37}$, F.~E.~Maas$^{15}$, M.~Maggiora$^{58A,58C}$, S.~Maldaner$^{26}$, S.~Malde$^{53}$, Q.~A.~Malik$^{57}$, A.~Mangoni$^{23B}$, Y.~J.~Mao$^{35}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{58A,58C}$, Z.~X.~Meng$^{49}$, J.~G.~Messchendorp$^{29}$, G.~Mezzadri$^{24A}$, J.~Min$^{1,43}$, T.~J.~Min$^{33}$, R.~E.~Mitchell$^{22}$, X.~H.~Mo$^{1,43,47}$, Y.~J.~Mo$^{6}$, C.~Morales Morales$^{15}$, N.~Yu.~Muchnoi$^{10,d}$, H.~Muramatsu$^{51}$, A.~Mustafa$^{4}$, S.~Nakhoul$^{11,g}$, Y.~Nefedov$^{27}$, F.~Nerling$^{11,g}$, I.~B.~Nikolaev$^{10,d}$, Z.~Ning$^{1,43}$, S.~Nisar$^{8,k}$, S.~L.~Niu$^{1,43}$, S.~L.~Olsen$^{47}$, Q.~Ouyang$^{1,43,47}$, S.~Pacetti$^{23B}$, Y.~Pan$^{55,43}$, M.~Papenbrock$^{59}$, P.~Patteri$^{23A}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{55,43}$, K.~Peters$^{11,g}$, J.~Pettersson$^{59}$, J.~L.~Ping$^{32}$, R.~G.~Ping$^{1,47}$, A.~Pitka$^{4}$, R.~Poling$^{51}$, V.~Prasad$^{55,43}$, M.~Qi$^{33}$, T.~Y.~Qi$^{2}$, S.~Qian$^{1,43}$, C.~F.~Qiao$^{47}$, N.~Qin$^{60}$, X.~P.~Qin$^{13}$, X.~S.~Qin$^{4}$, Z.~H.~Qin$^{1,43}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{34}$, K.~H.~Rashid$^{57,i}$, C.~F.~Redmer$^{26}$, M.~Richter$^{4}$, M.~Ripka$^{26}$, A.~Rivetti$^{58C}$, V.~Rodin$^{29}$, M.~Rolo$^{58C}$, G.~Rong$^{1,47}$, Ch.~Rosner$^{15}$, M.~Rump$^{52}$, A.~Sarantsev$^{27,e}$, M.~Savri\'e$^{24B}$, K.~Schoenning$^{59}$, W.~Shan$^{19}$, X.~Y.~Shan$^{55,43}$, M.~Shao$^{55,43}$, C.~P.~Shen$^{2}$, P.~X.~Shen$^{34}$, X.~Y.~Shen$^{1,47}$, H.~Y.~Sheng$^{1}$, X.~Shi$^{1,43}$, X.~D~Shi$^{55,43}$, J.~J.~Song$^{37}$, Q.~Q.~Song$^{55,43}$, X.~Y.~Song$^{1}$, S.~Sosio$^{58A,58C}$, C.~Sowa$^{4}$, S.~Spataro$^{58A,58C}$, F.~F. ~Sui$^{37}$, G.~X.~Sun$^{1}$, J.~F.~Sun$^{16}$, L.~Sun$^{60}$, S.~S.~Sun$^{1,47}$, X.~H.~Sun$^{1}$, Y.~J.~Sun$^{55,43}$, Y.~K~Sun$^{55,43}$, Y.~Z.~Sun$^{1}$, Z.~J.~Sun$^{1,43}$, Z.~T.~Sun$^{1}$, Y.~T~Tan$^{55,43}$, C.~J.~Tang$^{40}$, G.~Y.~Tang$^{1}$, X.~Tang$^{1}$, V.~Thoren$^{59}$, B.~Tsednee$^{25}$, I.~Uman$^{46D}$, B.~Wang$^{1}$, B.~L.~Wang$^{47}$, C.~W.~Wang$^{33}$, D.~Y.~Wang$^{35}$, H.~H.~Wang$^{37}$, K.~Wang$^{1,43}$, L.~L.~Wang$^{1}$, L.~S.~Wang$^{1}$, M.~Wang$^{37}$, M.~Z.~Wang$^{35}$, Meng~Wang$^{1,47}$, P.~L.~Wang$^{1}$, R.~M.~Wang$^{61}$, W.~P.~Wang$^{55,43}$, X.~Wang$^{35}$, X.~F.~Wang$^{1}$, X.~L.~Wang$^{9,j}$, Y.~Wang$^{44}$, Y.~Wang$^{55,43}$, Y.~F.~Wang$^{1,43,47}$, Z.~Wang$^{1,43}$, Z.~G.~Wang$^{1,43}$, Z.~Y.~Wang$^{1}$, Zongyuan~Wang$^{1,47}$, T.~Weber$^{4}$, D.~H.~Wei$^{12}$, P.~Weidenkaff$^{26}$, H.~W.~Wen$^{32}$, S.~P.~Wen$^{1}$, U.~Wiedner$^{4}$, G.~Wilkinson$^{53}$, M.~Wolke$^{59}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,47}$, Z.~Wu$^{1,43}$, L.~Xia$^{55,43}$, Y.~Xia$^{20}$, S.~Y.~Xiao$^{1}$, Y.~J.~Xiao$^{1,47}$, Z.~J.~Xiao$^{32}$, Y.~G.~Xie$^{1,43}$, Y.~H.~Xie$^{6}$, T.~Y.~Xing$^{1,47}$, X.~A.~Xiong$^{1,47}$, Q.~L.~Xiu$^{1,43}$, G.~F.~Xu$^{1}$, J.~J.~Xu$^{33}$, L.~Xu$^{1}$, Q.~J.~Xu$^{14}$, W.~Xu$^{1,47}$, X.~P.~Xu$^{41}$, F.~Yan$^{56}$, L.~Yan$^{58A,58C}$, W.~B.~Yan$^{55,43}$, W.~C.~Yan$^{2}$, Y.~H.~Yan$^{20}$, H.~J.~Yang$^{38,h}$, H.~X.~Yang$^{1}$, L.~Yang$^{60}$, R.~X.~Yang$^{55,43}$, S.~L.~Yang$^{1,47}$, Y.~H.~Yang$^{33}$, Y.~X.~Yang$^{12}$, Yifan~Yang$^{1,47}$, Z.~Q.~Yang$^{20}$, M.~Ye$^{1,43}$, M.~H.~Ye$^{7}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{44}$, B.~X.~Yu$^{1,43,47}$, C.~X.~Yu$^{34}$, J.~S.~Yu$^{20}$, C.~Z.~Yuan$^{1,47}$, X.~Q.~Yuan$^{35}$, Y.~Yuan$^{1}$, A.~Yuncu$^{46B,a}$, A.~A.~Zafar$^{57}$, Y.~Zeng$^{20}$, B.~X.~Zhang$^{1}$, B.~Y.~Zhang$^{1,43}$, C.~C.~Zhang$^{1}$, D.~H.~Zhang$^{1}$, H.~H.~Zhang$^{44}$, H.~Y.~Zhang$^{1,43}$, J.~Zhang$^{1,47}$, J.~L.~Zhang$^{61}$, J.~Q.~Zhang$^{4}$, J.~W.~Zhang$^{1,43,47}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,47}$, K.~Zhang$^{1,47}$, L.~Zhang$^{45}$, S.~F.~Zhang$^{33}$, T.~J.~Zhang$^{38,h}$, X.~Y.~Zhang$^{37}$, Y.~Zhang$^{55,43}$, Y.~H.~Zhang$^{1,43}$, Y.~T.~Zhang$^{55,43}$, Yang~Zhang$^{1}$, Yao~Zhang$^{1}$, Yi~Zhang$^{9,j}$, Yu~Zhang$^{47}$, Z.~H.~Zhang$^{6}$, Z.~P.~Zhang$^{55}$, Z.~Y.~Zhang$^{60}$, G.~Zhao$^{1}$, J.~W.~Zhao$^{1,43}$, J.~Y.~Zhao$^{1,47}$, J.~Z.~Zhao$^{1,43}$, Lei~Zhao$^{55,43}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{34}$, Q.~Zhao$^{1}$, S.~J.~Zhao$^{63}$, T.~C.~Zhao$^{1}$, Y.~B.~Zhao$^{1,43}$, Z.~G.~Zhao$^{55,43}$, A.~Zhemchugov$^{27,b}$, B.~Zheng$^{56}$, J.~P.~Zheng$^{1,43}$, Y.~Zheng$^{35}$, Y.~H.~Zheng$^{47}$, B.~Zhong$^{32}$, L.~Zhou$^{1,43}$, L.~P.~Zhou$^{1,47}$, Q.~Zhou$^{1,47}$, X.~Zhou$^{60}$, X.~K.~Zhou$^{47}$, X.~R.~Zhou$^{55,43}$, Xiaoyu~Zhou$^{20}$, Xu~Zhou$^{20}$, A.~N.~Zhu$^{1,47}$, J.~Zhu$^{34}$, J.~~Zhu$^{44}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,43,47}$, S.~H.~Zhu$^{54}$, W.~J.~Zhu$^{34}$, X.~L.~Zhu$^{45}$, Y.~C.~Zhu$^{55,43}$, Y.~S.~Zhu$^{1,47}$, Z.~A.~Zhu$^{1,47}$, J.~Zhuang$^{1,43}$, B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{8}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{9}$ Fudan University, Shanghai 200443, People's Republic of China\\
$^{10}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{11}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{12}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{13}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{14}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{15}$ Helmholtz Institute Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{16}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{17}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{18}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{19}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{20}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{21}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{22}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{23}$ (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN and University of Perugia, I-06100, Perugia, Italy\\
$^{24}$ (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{25}$ Institute of Physics and Technology, Peace Ave. 54B, Ulaanbaatar 13330, Mongolia\\
$^{26}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{27}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{28}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{29}$ KVI-CART, University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{30}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{31}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{32}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{33}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{34}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{35}$ Peking University, Beijing 100871, People's Republic of China\\
$^{36}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{37}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{38}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{39}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{40}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{41}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{42}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{43}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{44}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{45}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{46}$ (A)Ankara University, 06100 Tandogan, Ankara, Turkey; (B)Istanbul Bilgi University, 34060 Eyup, Istanbul, Turkey; (C)Uludag University, 16059 Bursa, Turkey; (D)Near East University, Nicosia, North Cyprus, Mersin 10, Turkey\\
$^{47}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{48}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{49}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{50}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{51}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
$^{52}$ University of Muenster, Wilhelm-Klemm-Str. 9, 48149 Muenster, Germany\\
$^{53}$ University of Oxford, Keble Rd, Oxford, UK OX13RH\\
$^{54}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{55}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{56}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{57}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{58}$ (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{59}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{60}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{61}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{62}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{63}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at Bogazici University, 34342 Istanbul, Turkey\\
$^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{c}$ Also at the Functional Electronics Laboratory, Tomsk State University, Tomsk, 634050, Russia\\
$^{d}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{e}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{f}$ Also at Istanbul Arel University, 34295 Istanbul, Turkey\\
$^{g}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{h}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{i}$ Also at Government College Women University, Sialkot - 51310. Punjab, Pakistan. \\
$^{j}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{k}$ Also at Harvard University, Department of Physics, Cambridge, MA, 02138, USA\\
}\end{center}

\vspace{0.4cm}
\end{small}

